Towards Unified Scene Text Spotting based on Sequence Generation

Sequence generation models have recently made significant progress in unifying various vision tasks. Although some auto-regressive models have demonstrated promising results in end-to-end text spotting, they use specific detection formats while ignoring various text shapes and are limited in the maximum number of text instances that can be detected. To overcome these limitations, we propose a UNIfied scene Text Spotter, called UNITS. Our model unifies various detection formats, including quadrilaterals and polygons, allowing it to detect text in arbitrary shapes. Additionally, we apply starting-point prompting to enable the model to extract texts from an arbitrary starting point, thereby extracting more texts beyond the number of instances it was trained on. Experimental results demonstrate that our method achieves competitive performance compared to state-of-the-art methods. Further analysis shows that UNITS can extract a larger number of texts than it was trained on. We provide the code for our method at https://github.com/clovaai/units.

==> supplemantal/suppl_spts.tex <==
{
\begin{table}
\centering
\begin{tabular}{lccc}
\toprule
\multirow{2}{*}{Method} & \multicolumn{2}{c}{End-to-End} \\
\cmidrule(lr){2-3}
                        & None & Full \\
\midrule
SPTS~\cite{peng2022spts}& 74.2 & 82.4 \\
\midrule
UNITS$_\textnormal{Shared}$ -- Point           & \textbf{78.2} & \textbf{86.7} \\
UNITS$_\textnormal{Shared}$ -- Box            & 77.9 & 86.6 \\
UNITS$_\textnormal{Shared}$ -- Quad           & 77.7 & 86.6 \\
UNITS$_\textnormal{Shared}$ -- Polygon        & 77.7 & 86.4 \\
\bottomrule
\end{tabular}
\caption{The end-to-end recognition performance evaluated by the point-based metric~\cite{peng2022spts} on Total-Text.}
\label{tab:exp_spts_totaltext}
\end{table}
}
